DeepVerge: Classification of Roadside Verge Biodiversity and Conservation Potential

Open space grassland is being increasingly farmed or built upon, leading to a ramping up of conservation efforts targeting roadside verges. Approximately half of all UK grassland species can be found along the country's 500,000 km of roads, with some 91 species either threatened or near threatened. Careful management of these "wildlife corridors" is therefore essential to preventing species extinction and maintaining biodiversity in grassland habitats. Wildlife trusts have often enlisted the support of volunteers to survey roadside verges and identify new "Local Wildlife Sites" as areas of high conservation potential. Using volunteer survey data from 3,900 km of roadside verges alongside publicly available street-view imagery, we present DeepVerge; a deep learning-based method that can automatically survey sections of roadside verges by detecting the presence of positive indicator species. Using images and ground truth survey data from the rural county of Lincolnshire, DeepVerge achieved a mean accuracy of 88%. Such a method may be used by local authorities to identify new local wildlife sites, and aid management and environmental planning in line with legal and government policy obligations, saving thousands of hours of manual labour.

==> cas-refs.old.tex <==
@ARTICLE{opensocietyC10,
    title={INFORMATION SHEET NO: C10 Highway Verges},
    author={Hornby-Steer, W. R.},
    year={2013},
    publisher={Open Spaces Society},
    institution={Open Spaces Society}
    }

@article{FULLER1987281,
title = {The changing extent and conservation interest of lowland grasslands in England and Wales: A review of grassland surveys 1930–1984},
journal = {Biological Conservation},
volume = {40},
number = {4},
pages = {281-300},
year = {1987},
issn = {0006-3207},
doi = {https://doi.org/10.1016/0006-3207(87)90121-2},
url = {https://www.sciencedirect.com/science/article/pii/0006320787901212},
author = {R.M. Fuller},
abstract = {This study has examined the changing extent of lowland grassland, in England and Wales, over the last half century. The proportions of semi-natural, and agriculturally improved grasslands were also assessed. Total grassland area has declined from 7·8 M ha, 50 years ago, to just 4·8 M ha now. The decline in extent of unimproved grasslands also started in the 1930s, accelerated through the war years, and has continued steadily ever since. The main agents, at first, were drainage and the plough. However, inorganic fertiliser use has increased simultaneously, improving even old unploughed grasslands. Only 0·6 M ha of semi-natural and rough grasslands remain in lowland England and Wales, making up only 11\% of the total grassland area. Semi-natural pastures excluding rough grasslands now cover only 0·2 M ha, 4\% of the present-day grassland area and 3\% of its area 50 years ago. Semi-natural pastures which survive have often seen some agricultural improvements, so that relatively few retain their conservation interest.}
}

@article{mazerolle2011google,
  title={Google Street View: a new online tool with potential application to roadside invasive species detection and monitoring},
  author={Mazerolle, David and Blaney, Sean},
  journal={PLANT INVASIONS},
  pages={77--83},
  year={2011},
  publisher={Citeseer}
}


@article{oshea_introduction_2015,
	title = {An {Introduction} to {Convolutional} {Neural} {Networks}},
	url = {http://arxiv.org/abs/1511.08458},
	abstract = {The field of machine learning has taken a dramatic twist in recent times, with the rise of the Artificial Neural Network (ANN). These biologically inspired computational models are able to far exceed the performance of previous forms of artificial intelligence in common machine learning tasks. One of the most impressive forms of ANN architecture is that of the Convolutional Neural Network (CNN). CNNs are primarily used to solve difficult image-driven pattern recognition tasks and with their precise yet simple architecture, offers a simplified method of getting started with ANNs. This document provides a brief introduction to CNNs, discussing recently published papers and newly formed techniques in developing these brilliantly fantastic image recognition models. This introduction assumes you are familiar with the fundamentals of ANNs and machine learning.},
	urldate = {2022-04-29},
	journal = {arXiv:1511.08458 [cs]},
	author = {O'Shea, Keiron and Nash, Ryan},
	month = dec,
	year = {2015},
	note = {arXiv: 1511.08458},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Computer Science - Neural and Evolutionary Computing},
	annote = {Comment: 10 pages, 5 figures},
	file = {arXiv Fulltext PDF:/home/andy/Zotero/storage/MQ2DAPYN/O'Shea and Nash - 2015 - An Introduction to Convolutional Neural Networks.pdf:application/pdf;arXiv.org Snapshot:/home/andy/Zotero/storage/HYJSZD9I/1511.html:text/html},
}


@ARTICLE{Plantlife2017,
    author = {Plantlife},
    title = {Road verges: Last refuge for some of our rarest wild flowers and plants},
    year = {2017},
    journal = { },
    institution = {Plantlife},
}

@ARTICLE{Biosphere2016,
title= {Life on the Verge – Biosphere Project 2016 – 2019: Independent Project Evaluation},
year = {2019},
author = {{David Rolls Associates}},
institution = {{David Rolls Associates}},
}

@ARTICLE{Plantlife2019,
    author = {Bromley, J. and McCarthy, B. and Shellswell, C.},
    title= {Managing grassland road verges: A best practice guide},
    year = {2019},
    journal = {},
    institution = {Plantlife}
}

@ARTICLE{UKNEA2011,
title= {Technical Report: The UK
National Ecosystem Assessment : Semi-natural Grasslands},
year = {2011},
author = {Richard G. Jefferson and Tim H. Blackstock and Robin J. Pakeman and Bridget A. Emmett and Richard J.
Pywell and J. Philip Grime and Jonathan Silvertown},
institution = {NERC Open Research Archive},
pages = {162-195}
}

@ARTICLE{CEH2007,
title= {Countryside Survey: UK Headline Messages from 2007},
year = {2008},
author = {P.D. Carey and S.M. Wallis and B.E. Emmett and L.C. Maskell and J. Murphy and L.R. Norton and I.C. Simpson and S.S. Smart},
institution = {Centre for Ecology \& Hydrology},
journal = {}
}

@article{RIDDING2015516,
title = {Fate of semi-natural grassland in England between 1960 and 2013: A test of national conservation policy},
journal = {Global Ecology and Conservation},
volume = {4},
pages = {516-525},
year = {2015},
issn = {2351-9894},
doi = {https://doi.org/10.1016/j.gecco.2015.10.004},
url = {https://www.sciencedirect.com/science/article/pii/S2351989415300184},
author = {Lucy E. Ridding and John W. Redhead and Richard F. Pywell},
keywords = {Grassland, Semi-natural, GIS, SSSI, Improved grassland, Agriculture},
abstract = {It is well documented that significant losses in semi-natural grassland occurred across Europe during the second half of the twentieth century. However, comparatively few studies have investigated and quantified the fate of large numbers of individual grassland areas. This is important for understanding the causes of decline, and consequently establishing new policies to conserve and restore lost habitats. This study addresses this problem; GIS was used to compare historic survey data collected between 1960 and 1981 with two contemporary spatial datasets of habitats in England. The datasets included the Priority Habitats Inventory 2013 and the Land Cover Map 2007 and this was undertaken for different types of semi-natural grassland across England. Considerable decreases occurred across the different grassland types, with a loss of 47\% of studied semi-natural grasslands sites in England over 32–53 years. Of this, the majority of grassland was lost to conversion to agriculturally-improved grassland or arable cultivation, 45\% and 43\% respectively. Changes to woodland and urban areas were also evident, but on a much smaller scale. Sites receiving statutory protection as a Site of Special Scientific Interest were found to have retained more grassland (91\%), compared with non-protected sites (27\%), thus highlighting the effectiveness of this aspect of current conservation policy in England, and the need for this to continue in the future.}
}

@article{Evans1,
author = {Evans, Michael J. and Malcom, Jacob W.},
title = {Supporting habitat conservation with automated change detection in Google Earth Engine},
journal = {Conservation Biology},
volume = {35},
number = {4},
pages = {1151-1161},
keywords = {Endangered Species Act, inventory and monitoring, land-cover change, politics and policy, remote sensing, threatened species, cambio en la cobertura del suelo, especies amenazadas, Ley de Especies en Peligro, inventario y monitoreo, políticas y normas, telemetría},
doi = {https://doi.org/10.1111/cobi.13680},
url = {https://conbio.onlinelibrary.wiley.com/doi/abs/10.1111/cobi.13680},
eprint = {https://conbio.onlinelibrary.wiley.com/doi/pdf/10.1111/cobi.13680},
abstract = {Abstract A significant limitation in biodiversity conservation has been the effective implementation of laws and regulations that protect species’ habitats from degradation. Flexible, efficient, and effective monitoring and enforcement methods are needed to help conservation policies realize their full benefit. As remote sensing data become more numerous and accessible, they can be used to identify and quantify land-cover changes and habitat loss. However, these data remain underused for systematic conservation monitoring in part because of a lack of simple tools. We adapted 2 algorithms that automatically identify differences between pairs of images. We used free, publicly available satellite data to evaluate their ability to rapidly detect land-cover changes in a variety of land-cover types. We compared algorithm predictions with ground-truthed results at 100 sites of known change in the United States. We also compared algorithm predictions to manually created polygons delineating anthropogenic change in 4 case studies involving imperiled species’ habitat: oil and gas development in the range of the Greater Sage Grouse (Centrocercus urophasianus); sand mining operations in the range of the dunes sagebrush lizard (Sceloporus arenicolus); loss of Piping Plover (Charadrius melodus) coastal habitat after Hurricane Michael (2018); and residential development in St. Andrew beach mouse (Peromyscus polionotus peninsularis) habitat. Both algorithms effectively discriminated between pixels corresponding to land-cover change and unchanged pixels as indicated by area under a receiver operating characteristic curve >0.90. The algorithm that was most effective differed among the case-study habitat types, and both effectively delineated habitat loss as indicated by low omission (min. = 0.0) and commission (min. = 0.0) rates, and moderate polygon overlap (max. = 47\%). Our results showed how these algorithms can be used to help close the implementation gap of monitoring and enforcement in biodiversity conservation. We provide a free online tool that can be used to run these analyses (https://conservationist.io/habitatpatrol).},
year = {2021}
}

@article{ROUSSELET2013,
title = {Assessing Species Distribution Using Google Street View: A Pilot Study with the Pine Processionary Moth},
journal = {PLoS ONE 8(10): e74918.},
volume = {8},
pages = {1-10},
year = {2013},
issn = {10},
doi = {https://doi.org/10.1371/journal.pone.0074918},
url = {https://journals.plos.org/plosone/article?id=10.1371/journal.pone.0074918},
author = {Jérôme Rousselet and Charles-Edouard Imbert and Anissa Dekri and Jacques Garcia and Francis Goussard and Bruno Vincent and Olivier Denux and Christelle Robinet and Franck Dorkeld and Alain Roques and Jean-Pierre Rossi }
}

@article{AINaturalists,
title = {AI Naturalists Might Hold the Key to Unlocking Biodiversity Data in Social Media Imagery},
journal = {Patterns},
volume = {1},
number = {7},
pages = {100116},
year = {2020},
issn = {2666-3899},
doi = {https://doi.org/10.1016/j.patter.2020.100116},
url = {https://www.sciencedirect.com/science/article/pii/S2666389920301574},
author = {Tom A. August and Oliver L. Pescott and Alexis Joly and Pierre Bonnet},
keywords = {artificial intelligence, computer vision, deep learning, machine learning, social media, biodiversity, informatics, botany, plants, big data},
abstract = {Summary
The increasing availability of digital images, coupled with sophisticated artificial intelligence (AI) techniques for image classification, presents an exciting opportunity for biodiversity researchers to create new datasets of species observations. We investigated whether an AI plant species classifier could extract previously unexploited biodiversity data from social media photos (Flickr). We found over 60,000 geolocated images tagged with the keyword “flower” across an urban and rural location in the UK and classified these using AI, reviewing these identifications and assessing the representativeness of images. Images were predominantly biodiversity focused, showing single species. Non-native garden plants dominated, particularly in the urban setting. The AI classifier performed best when photos were focused on single native species in wild situations but also performed well at higher taxonomic levels (genus and family), even when images substantially deviated from this. We present a checklist of questions that should be considered when undertaking a similar analysis.}
}

@article{JOHANSEN2019,
title = {Traditional semi-natural grassland management with heterogeneous mowing times enhances flower resources for pollinators in agricultural landscapes},
journal = {Global Ecology and Conservation},
volume = {18},
pages = {e00619},
year = {2019},
issn = {2351-9894},
doi = {https://doi.org/10.1016/j.gecco.2019.e00619},
url = {https://www.sciencedirect.com/science/article/pii/S2351989418303834},
author = {Line Johansen and Anna Westin and Sølvi Wehn and Anamaria Iuga and Cosmin Marius Ivascu and Eveliina Kallioniemi and Tommy Lennartsson},
keywords = {Wild pollinators, Semi-natural grassland, Traditional management, Floral resources, Phenological stage, Mowing time},
abstract = {For a diverse pollinator fauna it is important that pollen and nectar are available over the entire summer at spatially relevant scales. Semi-natural hay meadows are among the most important sources of flower resources for pollinators, but the resources are strongly affected by the timing of mowing. Management recommendations for hay meadows often prescribe late mowing on order to allow undisturbed flowering during most of the summer. Traditional practices, however, often include also earlier mowing. We investigate the link between the temporal variation of flower resources and traditional mowing practices of semi-natural hay meadows in a low-intensity agricultural landscape in Romania. In early August, we botanically surveyed meadows that were cut early, intermediately, or late in the season. We recorded all herb species, their phenological stage, and the number of reproductive units of each species. Data were analysed using DCA, LM and GLM. Plant species richness and composition are not affected by the time of mowing, but different sets of species flower in semi-natural grasslands with different mowing regimes. In August the proportion of species flowering and flower density are highest in the early-mown meadows due to re-flowering after mowing. Analyses of phenological stages indicate that late-mown meadows are the main pollen and nectar sources in July, whereas meadows mown early are the main resource from August to the end of the season. The results demonstrate that for pollinator conservation, heterogeneous mowing times within a landscape need to be encouraged when possible, and that strict focus on late mowing may lead to shortage of flower resources late in the summer. Studies of low-intensity agriculture has a great potential for learning about management methods that can be used in other parts of the world where traditional practices have been lost. Such studies can thereby contribute with important knowledge to manage global pollinator loss.}
}

@article{BARR200023,
title = {Estimating hedgerow length and pattern characteristics in Great Britain using Countryside Survey data},
journal = {Journal of Environmental Management},
volume = {60},
number = {1},
pages = {23-32},
year = {2000},
issn = {0301-4797},
doi = {https://doi.org/10.1006/jema.2000.0359},
url = {https://www.sciencedirect.com/science/article/pii/S0301479700903591},
author = {C.J Barr and M.K Gillespie},
keywords = {monitoring, connectedness, linear features, stock and change, hedgerow management, rural policy.},
abstract = {A chequer-board pattern of fields is characteristic of much of lowland Britain and other parts of western Europe. The field boundaries are often composed of hedgerows which, by tradition, are regularly managed to provide a relatively compact, sustainable, stock-proof barrier. The management regimes of hedgerows are, however, extremely variable resulting in a range of features, from low, compact, dense lines of shrubs through to tall, open rows of small trees. As well as providing an agronomic benefit, this network of several hundred thousand kilometres, has been shown to be a valuable resource to wildlife and is important as an aesthetic contribution to the British landscape. Therefore, the maintenance of the British hedgerow network is important and survey is essential to monitor its continuity. The Countryside Surveys have been used as means of achieving this, as well as providing a rich source of information, for example, about landscape pattern and changes in this over time. Hedgerow data have been collected during sample-based field surveys in 1978, 1984, 1990 and 1993. National estimates of the length of managed hedgerow derived from these data showed a 23\% reduction in the resource between 1984 and 1990. Much of this ‘loss’ appeared to be due to management regimes which have led to more overgrown hedgerows and rows of scattered shrubs. The proportion of mixed-species hedgerows increased between the two dates and there was a reduction in stockproof hedgerows but most other characteristics (e.g. height and management) remained constant. Landscape-pattern measures applied to the hedgerow network showed broad similarity across a range of landscape types in Britain although the density of hedges was greater in the pastural landscapes of the south and west. Measurement of ‘connectedness’, a feature of potential value in aiding species movement through the landscape, suggested that the British landscape is less-well connected in 1990 than previously. Hedgerows were found next to linear features, such as roads, as frequently as they were to any other land use. One of the most significant findings from analysis of 1984 and 1990 data was that there has been an increase in larger and more overgrown hedgerows, often to the point where they could no longer be defined as hedgerows. Overgrown hedgerows do have wildlife and other value but, to remain sustainable, hedgerows do require some degree of management. There is potential for using the Countryside Survey data further to provided better advice on the sustainable and sympathetic management of hedgerows. This is necessary to provide a rich and diverse network within a landscape or management unit. Countryside Survey hedgerow results have already been used to inform rural policy in Britain and have helped to underpin the introduction of policies and incentives which protect and enhance this landscape resource. These data are also being used to measure indicators of sustainable development and to provide a baseline against which changes in ancient and/or species-rich hedgerows can be assessed, as required in the UK Biodiversity Action Plan. The surveys have proved useful in gathering information on the hedgerows and other linear features in the British landscape. The approach could well be adapted to the needs of other countries where, for example, fencerows and roadside vegetation also provide an important ecological and landscape resource.}
}

@article{PHILLIPS2020108687,
title = {Enhancing road verges to aid pollinator conservation: A review},
journal = {Biological Conservation},
volume = {250},
pages = {108687},
year = {2020},
issn = {0006-3207},
doi = {https://doi.org/10.1016/j.biocon.2020.108687},
url = {https://www.sciencedirect.com/science/article/pii/S000632072030745X},
author = {Benjamin B. Phillips and Claire Wallace and Bethany R. Roberts and Andrew T. Whitehouse and Kevin J. Gaston and James M. Bullock and Lynn V. Dicks and Juliet L. Osborne},
keywords = {Roadside, Highway, Corridor, Roadkill, Pollution, Mowing, Insects, Bees, Butterflies, Moths, Flies, Beetles},
abstract = {Road verges provide habitats that have considerable potential as a tool for pollinator conservation, especially given the significant area of land that they collectively cover. Growing societal interest in managing road verges for pollinators suggests an immediate need for evidence-based management guidance. We used a formal, global literature review to assess evidence for the benefits of road verges for pollinators (as habitats and corridors), the potential negative impacts of roads on pollinators (vehicle-pollinator collisions, pollution, barriers to movement) and how to enhance road verges for pollinators through management. We identified, reviewed and synthesised 140 relevant studies. Overall, the literature review demonstrated that: (i) road verges are often hotspots of flowers and pollinators (well established), (ii) traffic and road pollution can cause mortality and other negative impacts on pollinators (well established), but available evidence suggests that the benefits of road verges to pollinators far outweigh the costs (established but incomplete), and (iii) road verges can be enhanced for pollinators through strategic management (well established). Future research should address the lack of holistic and large-scale understanding of the net effects of road verges on pollinators. We provide management recommendations for enhancing both individual road verges for pollinators (e.g. optimised mowing regimes) and entire road networks (e.g. prioritising enhancement of verges with the greatest capacity to benefit pollinators), and highlight three of the most strongly supported recommendations: (i) creating high quality habitats on new and existing road verges, (ii) reducing mowing frequency to 0–2 cuts/year and (iii) reducing impacts of street lighting.}
}

@article{biesmeijer2004parallel,
  title={Parallel Declines in Pollinators and Insect-Pollinated Plants in Britain and the Netherlands},
  author={Biesmeijer, JC and Roberts, SPM and Reemer, M and Ohlem{\"u}ller, R and Edwards, M and Peeters, T and Schaffers, AP and Potts, SG and Kleukers, R and Thomas, CD and others},
  journal={Microbiol. Immunol},
  volume={282},
  pages={1},
  year={2004}
}

@article{ILSVRC15,
Author = {Olga Russakovsky and Jia Deng and Hao Su and Jonathan Krause and Sanjeev Satheesh and Sean Ma and Zhiheng Huang and Andrej Karpathy and Aditya Khosla and Michael Bernstein and Alexander C. Berg and Li Fei-Fei},
Title = {{ImageNet Large Scale Visual Recognition Challenge}},
Year = {2015},
journal   = {International Journal of Computer Vision (IJCV)},
doi = {10.1007/s11263-015-0816-y},
volume={115},
number={3},
pages={211-252}
}

@article{DBLP:journals/corr/RazavianASC14,
  author    = {Ali Sharif Razavian and
               Hossein Azizpour and
               Josephine Sullivan and
               Stefan Carlsson},
  title     = {{CNN} Features off-the-shelf: an Astounding Baseline for Recognition},
  journal   = {CoRR},
  volume    = {abs/1403.6382},
  year      = {2014},
  url       = {http://arxiv.org/abs/1403.6382},
  eprinttype = {arXiv},
  eprint    = {1403.6382},
  timestamp = {Mon, 13 Aug 2018 16:46:52 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/RazavianASC14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{jain_artificial_1996,
	title = {Artificial neural networks: a tutorial},
	volume = {29},
	issn = {1558-0814},
	shorttitle = {Artificial neural networks},
	doi = {10.1109/2.485891},
	abstract = {Artificial neural nets (ANNs) are massively parallel systems with large numbers of interconnected simple processors. The article discusses the motivations behind the development of ANNs and describes the basic biological neuron and the artificial computational model. It outlines network architectures and learning processes, and presents some of the most commonly used ANN models. It concludes with character recognition, a successful ANN application.},
	number = {3},
	journal = {Computer},
	author = {Jain, A.K. and Mao, Jianchang and Mohiuddin, K.M.},
	month = mar,
	year = {1996},
	note = {Conference Name: Computer},
	keywords = {Artificial neural networks, Biological neural networks, Biological system modeling, Biology computing, Computer architecture, Concurrent computing, Humans, Integrated circuit interconnections, Parallel processing, Tutorial},
	pages = {31--44}
}


@article{deus_google_2016,
	title = {Google {Street} {View} as an alternative method to car surveys in large-scale vegetation assessments},
	volume = {188},
	issn = {1573-2959},
	url = {https://doi.org/10.1007/s10661-016-5555-1},
	doi = {10.1007/s10661-016-5555-1},
	abstract = {Car surveys (CS) are a common method for assessing the distribution of alien invasive plants. Google Street View (GSV), a free-access web technology where users may experience a virtual travel along roads, has been suggested as a cost-effective alternative to car surveys. We tested if we could replicate the results from a countrywide survey conducted by car in Portugal using GSV as a remote sensing tool, aiming at assessing the distribution of Eucalyptus globulus Labill. wildlings on roadsides adjacent to eucalypt stands. Georeferenced points gathered along CS were used to create road transects visible as lines overlapping the road in GSV environment, allowing surveying the same sampling areas using both methods. This paper presents the results of the comparison between the two methods. Both methods produced similar models of plant abundance, selecting the same explanatory variables, in the same hierarchical order of importance and depicting a similar influence on plant abundance. Even though the GSV model had a lower performance and the GSV survey detected fewer plants, additional variables collected exclusively with GSV improved model performance and provided a new insight into additional factors influencing plant abundance. The survey using GSV required ca. 9 \% of the funds and 62 \% of the time needed to accomplish the CS. We conclude that GSV may be a cost-effective alternative to CS. We discuss some advantages and limitations of GSV as a survey method. We forecast that GSV may become a widespread tool in road ecology, particularly in large-scale vegetation assessments.},
	language = {en},
	number = {10},
	urldate = {2022-04-21},
	journal = {Environmental Monitoring and Assessment},
	author = {Deus, Ernesto and Silva, Joaquim S. and Catry, Filipe X. and Rocha, Miguel and Moreira, Francisco},
	month = sep,
	year = {2016},
	keywords = {Alien invasive plants, Eucalypt, Remote sensing, Road ecology, Roadside, Wildling},
	pages = {560}
}


@ARTICAL{BIOTT2013,
title= {Life on the Verge: Wolds - HLF Evaluation Report},
year = {2013},
author = {Biott, E.},
institution = {Lincolnshire Wildlife Trust},
}

@report{Bot1933,
title= {THE BOTANICAL SOCIETY AND EXCHANGE CLUB OF THE BRITISH ISLES: REPORT FOR 1933. (VOL. X PART III},
year = {1934},
author = {William Harrison Pearsall},
institution = {The Botanical Society and Exchange Club of the British Isles},
}


@article{GSV,
author = {Anguelov, Dragomir and Dulong, Carole and Filip, Daniel and Frueh, Christian and Lafon, Stéphane and Lyon, Richard and Ogale, Abhijit and Vincent, Luc and Weaver, Josh},
year = {2010},
pages = {32-38},
title = {Google Street View: Capturing the World at Street Level},
volume = {43},
journal = {IEEE Computer},
doi = {10.1109/MC.2010.170}
}

@article{RINGLAND201936,
title = {Characterization of food cultivation along roadside transects with Google Street View imagery and deep learning},
journal = {Computers and Electronics in Agriculture},
volume = {158},
pages = {36-50},
year = {2019},
issn = {0168-1699},
doi = {https://doi.org/10.1016/j.compag.2019.01.014},
url = {https://www.sciencedirect.com/science/article/pii/S016816991831144X},
author = {John Ringland and Martha Bohm and So-Ra Baek},
keywords = {Google street view imagery, Computer vision or image classification, Food cultivation practices, Deep learning, Transfer learning, Convolutional neural network},
abstract = {We describe the development of tools to exploit the enormous resource of street-level imagery in Google Street View to characterize food cultivation practices along roadside transects at very high spatial resolution as a potential complement to traditional remote sensing approaches. We report on two software tools for crop identification using a deep convolutional neural network (CNN) applied to Google Street View imagery. The first, a multi-class classifier distinguishes seven regionally common cultivated plant species, as well as uncultivated vegetation, built environment, and water along the roads. The second, a prototype specialist detector, recognizes the presence of a single plant species: in our case, banana. These two classification tools were tested along roadside transects in two areas of Thailand, a country where there is good Google Street View coverage. On the entire test set, the overall accuracy of the multi-class classifier was 83.3\%. For several classes, (banana, built, cassava, maize, rice, and sugarcane), the producer's accuracy was over 90\%, meaning that the classifier was infrequently making omission errors. This performance on roadside transects is comparable with that of some remote-sensing classifiers, yet ours does not require any additional site-visits for ground-truthing. Moreover, the overall accuracy of the classifier on the 40\% of images it is most sure about is excellent: 99.0\%. For the prototype specialist detector, the area under the ROC curve was 0.9905, indicating excellent performance in detecting the presence of banana plants. While initially tested over the road network in a small area, this technique could readily be deployed on a regional or even national scale to supplement remote sensing data and yield a fine-grained analysis of food cultivation activities along roadside transects.}
}


@inproceedings{NIPS2014_b86e8d03,
 author = {Long, Jonathan L and Zhang, Ning and Darrell, Trevor},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {Z. Ghahramani and M. Welling and C. Cortes and N. Lawrence and K.Q. Weinberger},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Do Convnets Learn Correspondence?},
 url = {https://proceedings.neurips.cc/paper/2014/file/b86e8d03fe992d1b0e19656875ee557c-Paper.pdf},
 volume = {27},
 year = {2014}
}

@article{wei_understanding_2015,
	title = {Understanding {Intra}-{Class} {Knowledge} {Inside} {CNN}},
	url = {http://arxiv.org/abs/1507.02379},
	abstract = {Convolutional Neural Network (CNN) has been successful in image recognition tasks, and recent works shed lights on how CNN separates different classes with the learned inter-class knowledge through visualization [8, 10, 13]. In this work, we instead visualize the intra-class knowledge inside CNN to better understand how an object class is represented in the fully-connected layers. To invert the intraclass knowledge into more interpretable images, we propose a non-parametric patch prior upon previous CNN visualization models [8, 10]. With it, we show how different “styles” of templates for an object class are organized by CNN in terms of location and content, and represented in a hierarchical and ensemble way. Moreover, such intra-class knowledge can be used in many interesting applications, e.g. style-based image retrieval and style-based object completion.},
	language = {en},
	urldate = {2022-04-05},
	journal = {arXiv:1507.02379 [cs]},
	author = {Wei, Donglai and Zhou, Bolei and Torrabla, Antonio and Freeman, William},
	month = jul,
	year = {2015},
	note = {arXiv: 1507.02379},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	annote = {Comment: tech report for: http://vision03.csail.mit.edu/cnn\_art/index.html},
	file = {Wei et al. - 2015 - Understanding Intra-Class Knowledge Inside CNN.pdf:/home/andy/Zotero/storage/UVCWIW4H/Wei et al. - 2015 - Understanding Intra-Class Knowledge Inside CNN.pdf:application/pdf},
}


@article{chawla_smote_2002,
	title = {{SMOTE}: {Synthetic} {Minority} {Over}-sampling {Technique}},
	volume = {16},
	issn = {1076-9757},
	shorttitle = {{SMOTE}},
	url = {https://www.jair.org/index.php/jair/article/view/10302},
	doi = {10.1613/jair.953},
	abstract = {An approach to the construction of classiﬁers from imbalanced datasets is described. A dataset is imbalanced if the classiﬁcation categories are not approximately equally represented. Often real-world data sets are predominately composed of “normal” examples with only a small percentage of “abnormal” or “interesting” examples. It is also the case that the cost of misclassifying an abnormal (interesting) example as a normal example is often much higher than the cost of the reverse error. Under-sampling of the majority (normal) class has been proposed as a good means of increasing the sensitivity of a classiﬁer to the minority class. This paper shows that a combination of our method of over-sampling the minority (abnormal) class and under-sampling the majority (normal) class can achieve better classiﬁer performance (in ROC space) than only under-sampling the majority class. This paper also shows that a combination of our method of over-sampling the minority class and under-sampling the majority class can achieve better classiﬁer performance (in ROC space) than varying the loss ratios in Ripper or class priors in Naive Bayes. Our method of over-sampling the minority class involves creating synthetic minority class examples. Experiments are performed using C4.5, Ripper and a Naive Bayes classiﬁer. The method is evaluated using the area under the Receiver Operating Characteristic curve (AUC) and the ROC convex hull strategy.},
	language = {en},
	urldate = {2022-04-05},
	journal = {Journal of Artificial Intelligence Research},
	author = {Chawla, N. V. and Bowyer, K. W. and Hall, L. O. and Kegelmeyer, W. P.},
	month = jun,
	year = {2002},
	pages = {321--357},
	file = {Chawla et al. - 2002 - SMOTE Synthetic Minority Over-sampling Technique.pdf:/home/andy/Zotero/storage/89S8MV2A/Chawla et al. - 2002 - SMOTE Synthetic Minority Over-sampling Technique.pdf:application/pdf},
}


% CNNs

@misc{VTransformer,
  doi = {10.48550/ARXIV.2010.11929},
  url = {https://arxiv.org/abs/2010.11929},
  author = {Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and Uszkoreit, Jakob and Houlsby, Neil},
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
  publisher = {arXiv},
  year = {2020},
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{ConvNeXt,
  doi = {10.48550/ARXIV.2201.03545},
  url = {https://arxiv.org/abs/2201.03545},
  author = {Liu, Zhuang and Mao, Hanzi and Wu, Chao-Yuan and Feichtenhofer, Christoph and Darrell, Trevor and Xie, Saining},
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {A ConvNet for the 2020s},
  publisher = {arXiv},
  year = {2022},
  copyright = {Creative Commons Attribution 4.0 International}
}


@inproceedings{li_brief_2012,
	address = {Berlin, Heidelberg},
	title = {Brief {Introduction} of {Back} {Propagation} ({BP}) {Neural} {Network} {Algorithm} and {Its} {Improvement}},
	isbn = {978-3-642-30223-7},
	abstract = {The back propagation (BP) neural network algorithm is a multi-layer feedforward network trained according to error back propagation algorithm and is one of the most widely applied neural network models. BP network can be used to learn and store a great deal of mapping relations of input-output model, and no need to disclose in advance the mathematical equation that describes these mapping relations. Its learning rule is to adopt the steepest descent method in which the back propagation is used to regulate the weight value and threshold value of the network to achieve the minimum error sum of square. This paper focuses on the analysis of the characteristics and mathematical theory of BP neural network and also points out the shortcomings of BP algorithm as well as several methods for improvement.},
	booktitle = {Advances in {Computer} {Science} and {Information} {Engineering}},
	publisher = {Springer Berlin Heidelberg},
	author = {Li, Jing and Cheng, Ji-hang and Shi, Jing-yuan and Huang, Fei},
	editor = {Jin, David and Lin, Sally},
	year = {2012},
	pages = {553--558},
}

@article{dumoulin_guide_2018,
	title = {A guide to convolution arithmetic for deep learning},
	url = {http://arxiv.org/abs/1603.07285},
	abstract = {We introduce a guide to help deep learning practitioners understand and manipulate convolutional neural network architectures. The guide clarifies the relationship between various properties (input shape, kernel shape, zero padding, strides and output shape) of convolutional, pooling and transposed convolutional layers, as well as the relationship between convolutional and transposed convolutional layers. Relationships are derived for various cases, and are illustrated in order to make them intuitive.},
	urldate = {2022-05-03},
	journal = {arXiv:1603.07285 [cs, stat]},
	author = {Dumoulin, Vincent and Visin, Francesco},
	month = jan,
	year = {2018},
	note = {arXiv: 1603.07285},
	keywords = {Computer Science - Machine Learning, Computer Science - Neural and Evolutionary Computing, Statistics - Machine Learning}
}


@inproceedings{ioffe_batch_2015,
	title = {Batch {Normalization}: {Accelerating} {Deep} {Network} {Training} by {Reducing} {Internal} {Covariate} {Shift}},
	shorttitle = {Batch {Normalization}},
	url = {https://proceedings.mlr.press/v37/ioffe15.html},
	abstract = {Training Deep Neural Networks is complicated by the fact that the distribution of each layer’s inputs changes during training, as the parameters of the previous layers change. This slows down the training by requiring lower learning rates and careful parameter initialization, and makes it notoriously hard to train models with saturating nonlinearities. We refer to this phenomenon as internal covariate shift, and address the problem by normalizing layer inputs. Our method draws its strength from making normalization a part of the model architecture and performing the normalization for each training mini-batch. Batch Normalization allows us to use much higher learning rates and be less careful about initialization, and in some cases eliminates the need for Dropout. Applied to a stateof-the-art image classification model, Batch Normalization achieves the same accuracy with 14 times fewer training steps, and beats the original model by a significant margin. Using an ensemble of batch-normalized networks, we improve upon the best published result on ImageNet classification: reaching 4.82\% top-5 test error, exceeding the accuracy of human raters.},
	language = {en},
	urldate = {2022-05-06},
	booktitle = {Proceedings of the 32nd {International} {Conference} on {Machine} {Learning}},
	publisher = {PMLR},
	author = {Ioffe, Sergey and Szegedy, Christian},
	month = jun,
	year = {2015},
	note = {ISSN: 1938-7228},
	pages = {448--456}
}


@article{sun_ampnet_2021,
	title = {{AMPNet}: {Average}- and {Max}-{Pool} {Networks} for {Salient} {Object} {Detection}},
	volume = {31},
	issn = {1558-2205},
	shorttitle = {{AMPNet}},
	doi = {10.1109/TCSVT.2021.3054471},
	abstract = {Salient Object Detection aims to detect the most visually distinctive objects in an image. We solve this problem by introducing the average pool to explore the multi-level deep average pool convolution features different from the max pool information. Based on the U-net structure, we propose an Average- and Max-Pool Network (AMPNet) that leverages the average- and max-pool modules to integrate the multi-level complementary contextual features in the spatial and channel-wise dimensions, respectively. The complementary contextual features generated by our network can improve the completeness of detected objects. It has been observed that the non-salient regions are misrecognized as the salient objects because of the redundant information contained in the multi-level convolution features. To address the problem, two top-down feedback paths are introduced based on the above two modules, and their top-level semantic guidance information is fully utilized to improve the accuracy of salient objects detection. Finally, we apply the Feature Fusion Module and Deep Supervision Mechanism to further improve the performance of the network over different datasets. Experimental results on six benchmark datasets show that our network is on par with state-of-the-art approaches. Our method runs at more than 45 FPS (based on VGG) and 35 FPS (based on ResNet) on a single GPU and meets real-time requirements.},
	number = {11},
	journal = {IEEE Transactions on Circuits and Systems for Video Technology},
	author = {Sun, Luna and Chen, Zhenxue and Wu, Q. M. Jonathan and Zhao, Hongjian and He, Weikai and Yan, Xinghe},
	month = nov,
	year = {2021},
	note = {Conference Name: IEEE Transactions on Circuits and Systems for Video Technology},
	keywords = {Average pool, Convolution, Feature extraction, max pool, Neural networks, Object detection, salient object detection, Semantics, Task analysis, two top-down paths, Visualization},
	pages = {4321--4333}
}


@article{agarap_deep_2019,
	title = {Deep {Learning} using {Rectified} {Linear} {Units} ({ReLU})},
	url = {http://arxiv.org/abs/1803.08375},
	abstract = {We introduce the use of rectified linear units (ReLU) as the classification function in a deep neural network (DNN). Conventionally, ReLU is used as an activation function in DNNs, with Softmax function as their classification function. However, there have been several studies on using a classification function other than Softmax, and this study is an addition to those. We accomplish this by taking the activation of the penultimate layer \$h\_\{n - 1\}\$ in a neural network, then multiply it by weight parameters \${\textbackslash}theta\$ to get the raw scores \$o\_\{i\}\$. Afterwards, we threshold the raw scores \$o\_\{i\}\$ by \$0\$, i.e. \$f(o) = {\textbackslash}max(0, o\_\{i\})\$, where \$f(o)\$ is the ReLU function. We provide class predictions \${\textbackslash}hat\{y\}\$ through argmax function, i.e. argmax \$f(x)\$.},
	urldate = {2022-05-05},
	journal = {arXiv:1803.08375 [cs, stat]},
	author = {Agarap, Abien Fred},
	month = feb,
	year = {2019},
	note = {arXiv: 1803.08375},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Computer Science - Neural and Evolutionary Computing, Statistics - Machine Learning},
	annote = {Comment: 7 pages, 11 figures, 9 tables}
}


@article{EfficientNet,
  doi = {10.48550/ARXIV.1905.11946},
  url = {https://arxiv.org/abs/1905.11946},
  author = {Tan, Mingxing and Le, Quoc V.},
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {EfficientNet: Rethinking Model Scaling for Convolutional Neural Networks},
  publisher = {arXiv},
  year = {2019},
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{BILJECKI2021104217,
title = {Street view imagery in urban analytics and GIS: A review},
journal = {Landscape and Urban Planning},
volume = {215},
pages = {104217},
year = {2021},
issn = {0169-2046},
doi = {https://doi.org/10.1016/j.landurbplan.2021.104217},
url = {https://www.sciencedirect.com/science/article/pii/S0169204621001808},
author = {Filip Biljecki and Koichi Ito},
keywords = {Urban data science, Urban planning, Built environment, Deep learning, Remote sensing, Ground-level},
abstract = {Street view imagery has rapidly ascended as an important data source for geospatial data collection and urban analytics, deriving insights and supporting informed decisions. Such surge has been mainly catalysed by the proliferation of large-scale imagery platforms, advances in computer vision and machine learning, and availability of computing resources. We screened more than 600 recent papers to provide a comprehensive systematic review of the state of the art of how street-level imagery is currently used in studies pertaining to the built environment. The main findings are that: (i) street view imagery is now clearly an entrenched component of urban analytics and GIScience; (ii) most of the research relies on data from Google Street View; and (iii) it is used across myriads of domains with numerous applications – ranging from analysing vegetation and transportation to health and socio-economic studies. A notable trend is crowdsourced street view imagery, facilitated by services such as Mapillary and KartaView, in some cases furthering geographical coverage and temporal granularity, at a permissive licence.}
}

@article{kotowska_evaluating_2021,
	title = {Evaluating {Google} {Street} {View} for tracking invasive alien plants along roads},
	volume = {121},
	issn = {1470160X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S1470160X20309596},
	doi = {10.1016/j.ecolind.2020.107020},
	abstract = {Invasive alien plants are considered a major driver of global biodiversity loss. Therefore, there is a huge demand of spatial and temporal data on their distribution for investigating possible drivers of species invasions and for predictions of future distributions. We use Google Street View imagery (GSV) as a new source of spatial and temporal data. GSV provides millions of panoramic views along road networks worldwide allowing for the identification of many plant species, including invasive ones. Thus, GSV has a great potential to support ecological research in documenting species distribution, but reliable validation of its precision and accuracy is lacking. Here, we describe and evaluate an approach using GSV to visually track the spread of invasive alien plants, the North American goldenrods (Solidago canadensis and S. gigantea) occurring abundantly along road network in Poland (Central Europe). We determined presence/absence of the species along 160 randomly selected transects of a length of 500 m by visual inspection of GSV images and compared it with field surveys at the same transects. We show that the occurrence of goldenrods in GSV is a reliable predictor of their occurrence in the wild. Sampling parameters, like road width, season when GSV pictures were taken and number of months elapsed since taking the GSV pictures, did not change the correlation between outputs of the two methods (GSV and field sampling). Furthermore, both the occurrence of goldenrods observed in the field and their occurrence in GSV have similar relations to habitat characteristics investigated (the same direction of relationship and similar effect size). We suggest Google Street View images may be an additional tool to be used in the detection and tracking of the spread of invasive alien plants along roadsides. The approach may be useful in assessing temporal changes in roadside vegetation and managing problematic plant species across large spatial scales and may contribute to the further development of more efficient sampling methods in ecological studies.},
	language = {en},
	urldate = {2022-04-05},
	journal = {Ecological Indicators},
	author = {Kotowska, Dorota and Pärt, Tomas and Żmihorski, Michał},
	month = feb,
	year = {2021},
	pages = {107020},
	file = {Kotowska et al. - 2021 - Evaluating Google Street View for tracking invasiv.pdf:/home/andy/Zotero/storage/8DHW7LJU/Kotowska et al. - 2021 - Evaluating Google Street View for tracking invasiv.pdf:application/pdf},
}

@article{depauw_use_nodate,
	title = {The use of photos to investigate ecological change},
	volume = {n/a},
	issn = {1365-2745},
	url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/1365-2745.13876},
	doi = {10.1111/1365-2745.13876},
	year = {2022},
	abstract = {Global change is causing ecosystems to change at unprecedented rates and the urgency to quantify ecological change is high. We therefore need all possible sources of ecological data to address key knowledge gaps. Ground-based photos are a form of remote sensing and an unconventional data source with a high potential to improve our understanding of ecological change. They can provide invaluable information on ecological conditions in the past and present at relevant spatiotemporal scales that is very difficult to obtain with other approaches. Here we review the use of ground-based photos in a set of relevant ecological research topics, such as biodiversity and community ecology, phenology, global change ecology and landscape ecology. We highlight three main photo-based methods in ecological research (repeat photography, time-lapse photography and public archives), alongside which we discuss three case studies to demonstrate novel applications of these methods, to answer fundamental ecological questions. Synthesis. Photos can significantly support ecological research to improve our understanding of biotic responses in a rapidly changing world. Photos cover relatively large temporal and spatial scales, and can provide large amounts of information with limited time investment. To exploit their full potential, we need to invest not only in technological advances to compile, process and analyse images but also in proper data management.},
	language = {en},
	number = {n/a},
	urldate = {2022-04-17},
	journal = {Journal of Ecology},
	author = {Depauw, Leen and Blondeel, Haben and De Lombaerde, Emiel and De Pauw, Karen and Landuyt, Dries and Lorer, Eline and Vangansbeke, Pieter and Vanneste, Thomas and Verheyen, Kris and De Frenne, Pieter},
	note = {\_eprint: https://onlinelibrary.wiley.com/doi/pdf/10.1111/1365-2745.13876},
	keywords = {ecological change, Google Street View, ground-based photography, iEcology, plant ecology, remote sensing, repeat photography, time-lapse photography},
}

% Augmentation


@inproceedings{li_simple_2021,
	title = {A {Simple} {Feature} {Augmentation} for {Domain} {Generalization}},
	url = {https://openaccess.thecvf.com/content/ICCV2021/html/Li_A_Simple_Feature_Augmentation_for_Domain_Generalization_ICCV_2021_paper.html},
	language = {en},
	urldate = {2022-05-03},
	author = {Li, Pan and Li, Da and Li, Wei and Gong, Shaogang and Fu, Yanwei and Hospedales, Timothy M.},
	year = {2021},
	pages = {8886--8895}
}



@article{shorten_survey_2019,
	title = {A survey on {Image} {Data} {Augmentation} for {Deep} {Learning}},
	volume = {6},
	issn = {2196-1115},
	url = {https://doi.org/10.1186/s40537-019-0197-0},
	doi = {10.1186/s40537-019-0197-0},
	abstract = {Deep convolutional neural networks have performed remarkably well on many Computer Vision tasks. However, these networks are heavily reliant on big data to avoid overfitting. Overfitting refers to the phenomenon when a network learns a function with very high variance such as to perfectly model the training data. Unfortunately, many application domains do not have access to big data, such as medical image analysis. This survey focuses on Data Augmentation, a data-space solution to the problem of limited data. Data Augmentation encompasses a suite of techniques that enhance the size and quality of training datasets such that better Deep Learning models can be built using them. The image augmentation algorithms discussed in this survey include geometric transformations, color space augmentations, kernel filters, mixing images, random erasing, feature space augmentation, adversarial training, generative adversarial networks, neural style transfer, and meta-learning. The application of augmentation methods based on GANs are heavily covered in this survey. In addition to augmentation techniques, this paper will briefly discuss other characteristics of Data Augmentation such as test-time augmentation, resolution impact, final dataset size, and curriculum learning. This survey will present existing methods for Data Augmentation, promising developments, and meta-level decisions for implementing Data Augmentation. Readers will understand how Data Augmentation can improve the performance of their models and expand limited datasets to take advantage of the capabilities of big data.},
	language = {en},
	number = {1},
	urldate = {2022-05-03},
	journal = {Journal of Big Data},
	author = {Shorten, Connor and Khoshgoftaar, Taghi M.},
	month = jul,
	year = {2019},
	keywords = {Big data, Data Augmentation, Deep Learning, GANs, Image data},
	pages = {60}
}


@article{perez_effectiveness_2017,
	title = {The {Effectiveness} of {Data} {Augmentation} in {Image} {Classification} using {Deep} {Learning}},
	url = {http://arxiv.org/abs/1712.04621},
	abstract = {In this paper, we explore and compare multiple solutions to the problem of data augmentation in image classification. Previous work has demonstrated the effectiveness of data augmentation through simple techniques, such as cropping, rotating, and flipping input images. We artificially constrain our access to data to a small subset of the ImageNet dataset, and compare each data augmentation technique in turn. One of the more successful data augmentations strategies is the traditional transformations mentioned above. We also experiment with GANs to generate images of different styles. Finally, we propose a method to allow a neural net to learn augmentations that best improve the classifier, which we call neural augmentation. We discuss the successes and shortcomings of this method on various datasets.},
	urldate = {2022-05-03},
	journal = {arXiv:1712.04621 [cs]},
	author = {Perez, Luis and Wang, Jason},
	month = dec,
	year = {2017},
	note = {arXiv: 1712.04621},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	annote = {Comment: 8 pages, 12 figures}
}


@techreport{neil_local_2013,
	title = {Local {Wildlife} {Site} {Guidelines} for {Greater} {Lincolnshire}},
	url = {https://glnp.org.uk/images/uploads/services/5e84eae57f8a5_LWS%20guidelines%203rd%20ed.pdf},
	language = {en},
	number = {3rd edition},
	urldate = {2022-04-16},
	institution = {Greater Lincolnshire Nature Partnership},
	author = {Neil, Pike},
	year = {2013},
	pages = {114}
}

% Grid / interval GSV extraction

@article{nguyen_using_2020,
	title = {Using 164 {Million} {Google} {Street} {View} {Images} to {Derive} {Built} {Environment} {Predictors} of {COVID}-19 {Cases}},
	volume = {17},
	issn = {1660-4601},
	url = {https://www.mdpi.com/1660-4601/17/17/6359},
	doi = {10.3390/ijerph17176359},
	abstract = {The spread of COVID-19 is not evenly distributed. Neighborhood environments may structure risks and resources that produce COVID-19 disparities. Neighborhood built environments that allow greater ﬂow of people into an area or impede social distancing practices may increase residents’ risk for contracting the virus. We leveraged Google Street View (GSV) images and computer vision to detect built environment features (presence of a crosswalk, non-single family home, single-lane roads, dilapidated building and visible wires). We utilized Poisson regression models to determine associations of built environment characteristics with COVID-19 cases. Indicators of mixed land use (non-single family home), walkability (sidewalks), and physical disorder (dilapidated buildings and visible wires) were connected with higher COVID-19 cases. Indicators of lower urban development (single lane roads and green streets) were connected with fewer COVID-19 cases. Percent black and percent with less than a high school education were associated with more COVID-19 cases. Our ﬁndings suggest that built environment characteristics can help characterize community-level COVID-19 risk. Sociodemographic disparities also highlight diﬀerential COVID-19 risk across groups of people. Computer vision and big data image sources make national studies of built environment eﬀects on COVID-19 risk possible, to inform local area decision-making.},
	language = {en},
	number = {17},
	urldate = {2022-04-05},
	journal = {International Journal of Environmental Research and Public Health},
	author = {Nguyen, Quynh C. and Huang, Yuru and Kumar, Abhinav and Duan, Haoshu and Keralis, Jessica M. and Dwivedi, Pallavi and Meng, Hsien-Wen and Brunisholz, Kimberly D. and Jay, Jonathan and Javanmardi, Mehran and Tasdizen, Tolga},
	month = sep,
	year = {2020},
	pages = {6359},
	file = {Nguyen et al. - 2020 - Using 164 Million Google Street View Images to Der.pdf:/home/andy/Zotero/storage/U9IBF5GR/Nguyen et al. - 2020 - Using 164 Million Google Street View Images to Der.pdf:application/pdf},
}

@article{kim_decoding_2021,
	title = {Decoding urban landscapes: {Google} street view and measurement sensitivity},
	volume = {88},
	issn = {01989715},
	shorttitle = {Decoding urban landscapes},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0198971521000338},
	doi = {10.1016/j.compenvurbsys.2021.101626},
	abstract = {While Google Street View (GSV) has been increasingly available for large-scale examinations of urban land­ scapes, little is known about how to use this promising data source more cautiously and effectively. Using data for Santa Ana, California, as an example, this study provides an empirical assessment of the sensitivity of GSVbased streetscape measures and their variation patterns. The results show that the measurement outcomes can vary substantially with changes in GSV acquisition parameter settings, specifically spacing and direction. The sensitivity is found to be particularly high for some measurement targets, including humans, objects, and sidewalks. Some of these elements, such as buildings and sidewalks, also show highly correlated patterns of variation indicating their covariance in the mosaic of urban space.},
	language = {en},
	urldate = {2022-04-05},
	journal = {Computers, Environment and Urban Systems},
	author = {Kim, Jae Hong and Lee, Sugie and Hipp, John R. and Ki, Donghwan},
	month = jul,
	year = {2021},
	pages = {101626},
	file = {Kim et al. - 2021 - Decoding urban landscapes Google street view and .pdf:/home/andy/Zotero/storage/3NES2XG8/Kim et al. - 2021 - Decoding urban landscapes Google street view and .pdf:application/pdf},
}


@article{stubbings_hierarchical_2019,
	title = {A {Hierarchical} {Urban} {Forest} {Index} {Using} {Street}-{Level} {Imagery} and {Deep} {Learning}},
	volume = {11},
	issn = {2072-4292},
	url = {https://www.mdpi.com/2072-4292/11/12/1395},
	doi = {10.3390/rs11121395},
	abstract = {We develop a method based on computer vision and a hierarchical multilevel model to derive an Urban Street Tree Vegetation Index which aims to quantify the amount of vegetation visible from the point of view of a pedestrian. Our approach unfolds in two steps. First, areas of vegetation are detected within street-level imagery using a state-of-the-art deep neural network model. Second, information is combined from several images to derive an aggregated indicator at the area level using a hierarchical multilevel model. The comparative performance of our proposed approach is demonstrated against a widely used image segmentation technique based on a pre-labelled dataset. The approach is deployed to a real-world scenario for the city of Cardiff, Wales, using Google Street View imagery. Based on more than 200,000 street-level images, an urban tree street-level indicator is derived to measure the spatial distribution of tree cover, accounting for the presence of obstructing objects present in images at the Lower Layer Super Output Area (LSOA) level, corresponding to the most commonly used administrative areas for policy-making in the United Kingdom. The results show a high degree of correspondence between our tree street-level score and aerial tree cover estimates. They also evidence more accurate estimates at a pedestrian perspective from our tree score by more appropriately capturing tree cover in areas with large burial, woodland, formal open and informal open spaces where shallow trees are abundant, in high density residential areas with backyard trees, and along street networks with high density of high trees. The proposed approach is scalable and automatable. It can be applied to cities across the world and provides robust estimates of urban trees to advance our understanding of the link between mental health, well-being, green space and air pollution.},
	language = {en},
	number = {12},
	urldate = {2022-04-05},
	journal = {Remote Sensing},
	author = {Stubbings, Philip and Peskett, Joe and Rowe, Francisco and Arribas-Bel, Dani},
	month = jun,
	year = {2019},
	pages = {1395},
	file = {Stubbings et al. - 2019 - A Hierarchical Urban Forest Index Using Street-Lev.pdf:/home/andy/Zotero/storage/EEUCCEP6/Stubbings et al. - 2019 - A Hierarchical Urban Forest Index Using Street-Lev.pdf:application/pdf},
}



@article{warzecha2018attractiveness,
  title={Attractiveness of wildflower mixtures for wild bees and hoverflies depends on some key plant species},
  author={Warzecha, Daniela and Diek{\"o}tter, Tim and Wolters, Volkmar and Jauker, Frank},
  journal={Insect Conservation and Diversity},
  volume={11},
  number={1},
  pages={32--41},
  year={2018},
  publisher={Wiley Online Library}
}

@phdthesis{FriedlandPhdthesis,
  author  = {Friedland, Carol J.},
  title   = {Residential building damage from hurricane storm surge: proposed methodologies to describe, assess and model building damage},
  school  = {Louisiana State University and Agricultural and Mechanical College},
  address = {Louisiana , USA},
  year    = {2009}
}



% ANDY Added

@online{Wildlifetrusts1,
    author= {{The Wildlife Trusts}},
    year  = {2019},
    publisher = {The Wildlife Trusts},
    title = {Managing road verges: An introduction to the basics of managing road verges for wildlife},
    note  = { Newark: The Wildlife Trusts. Available from \url{ https://www.wildlifetrusts.org/wildlife/managing-land-wildlife/managing-road-verges-wildlife} 
             [accessed 17 Feb 2022].},
}


@online{Gov1,
    author= {{Gov.UK}},
    year  = {2021},
    publisher = {Department for Environment, Food \& Rural Affairs and Rural Payments Agency},
    title = {Guidance: Improved grassland standard of the Sustainable Farming Incentive pilot},
    note  = { London: Department for Environment, Food \& Rural Affairs and Rural Payments Agency. Available from \url{ https://www.gov.uk/guidance/improved-grassland-standard} 
             [accessed 17 Feb 2022].},
}



@online{LWT1,
    author= {{Lincolnshire Wildlife Trust}},
    year  = {2021},
    publisher = {Lincolnshire Wildlife Trust},
    title = {Lincolnshire Wildlife Trust},
    note  = { Horncastle, UK: Lincolnshire Wildlife Trust. Available from \url{ https://www.lincstrust.org.uk/} 
             [accessed 17 Feb 2022].},
}

@online{LWT2,
    author= {{Lincolnshire Wildlife Trust}},
    year  = {2021},
    publisher = {Lincolnshire Wildlife Trust},
    title = {Roadside Biomass Harvesting FAQ},
    note  = { Horncastle, UK: Lincolnshire Wildlife Trust. Available from \url{ https://www.lincstrust.org.uk/wildlife/wildlife-gardening/wildflower-hub/verges-faq} 
             [accessed 17 Feb 2022].},
}

@online{LotV1,
    author= {{Lincolnshire Wildlife Trust}},
    year  = {2016},
    publisher = {Lincolnshire Wildlife Trust},
    title = {Life on the Verge},
    note  = { Horncastle, UK: Lincolnshire Wildlife Trust. Available from \url{ https://www.lincstrust.org.uk/what-we-do/wildlife-conservation/projects/life-on-the-verge} 
             [accessed 17 Feb 2022].},
}

@online{LotV2013,
    author= {{Lincolnshire Wildlife Trust}},
    year  = {2013},
    publisher = {Lincolnshire Wildlife Trust},
    title = {Life on the Verge},
    note  = { Horncastle, UK: Lincolnshire Wildlife Trust. Available from \url{http://www.lifeontheverge.org.uk/} 
             [accessed 9 Mar 2022].},
}

@online{Devon1,
    author= {{Devon County Council}},
    year  = {2021},
    publisher = {Devon County Council},
    title = {Devon County Council},
    note  = { Devon, UK: Devon County Council. Available from \url{ https://www.devon.gov.uk/environment/wildlife/managing-verges-for-wildlife} 
             [accessed 17 Feb 2022].},
}

@online{Biosphere1,
    author= {{Tarka Country Trust}},
    year  = {2020},
    publisher = {Tarka Country Trust},
    title = {Life On The Verge - Biosphere (2016 - 2020)},
    note  = { Barnstable, UK: Tarka Country Trust. Available from \url{ https://www.tarkacountrytrust.org.uk/love-b-883968.html} [accessed 17 Feb 2022].},
}

@online{OGC1,
    author= {{Open Geospatial Consortium}},
    year  = {2020},
    publisher = {Open Geospatial Consortium},
    title = {KML},
    note  = { Arlington, USA: Open Geospatial Consortium. Available from \url{https://www.ogc.org/standards/kml} [accessed 6 Mar 2022].},
}

@online{ERSI1,
    author= {{Esri (UK) Ltd}},
    year  = {2011},
    publisher = {Esri (UK) Ltd},
    title = {Keyhole Markup Language},
    note  = { London, UK: Esri (UK) Ltd. Available from \url{http://wiki.gis.com/wiki/index.php/Keyhole_Markup_Language} [accessed 6 Mar 2022].},
}

==> text-scraps.tex <==
\subsection{Convolutional Neural Networks}
A CNN extracts learnable image features from a labelled image by sliding a pixel filter matrix (a kernel with a width and height) across the entire image in regular sized steps (called strides). The filter is convolved with the part of the image at the stepped filter position, producing an approximation of the filtered image area using the mathematical dot product. After the filter has been stepped across the entire image an overall generalisation of that image will be produced. Each filtered area has, in effect, extracted the key \emph{feature} that describes that area. The collection of \emph{feature areas} form a feature map of the original image. Multiple feature maps can be produced by multiple filters, which can then be generalised further by \emph{pooling} together features to reduce the amount of information.

The process can be repeated in layers, or blocks of repeated convolutions, with each block reducing the image width and height, while at the same time increasing the depth of the feature maps (channels) using different filters. The resulting array of feature maps can then be translated into a one to one mapping between the convolution output and the input of a Fully Connected Neural Network (FCNN). The original image's features are in effect fed through the CNN algorithm and a correlation between the features and the image's label is attempted using statistical probabilities. How probable the features are correlated to the label gives rise to a size of error metric at the FCNN output. A proportion of the error is then fed back (back propagated) through the network to change the filter's parameters, and the whole process is repeated until the process reduces the error as far as is possible. The filter parameters are thereby determined (learned) as a way to find the best filter that can recognise generalised patterns of features that best describe the image.  

Images will be taken from these locations, annotated with the score, taking care to reduce noise caused by false labelling, producing the GT dataset. 

Any number of sub-datasets can be produced by selecting or targeting specific locations, dates the panoramic views were taken, the perspective, camera pitch and zoom level of each image. Each location can also have multiple images taken from different perspectives to increase the dataset samples. \petra{Unclear. Let's discuss.}

As seen in Fig \ref{fig:RoadGrid}, whether a grid is used or simply requesting images every x metres, GSV will return the \emph{snapped to} panorama which relates to the area that the GPS requested image falls within.
